Cutting through form factors and cross sections of non-protected operators in N=4 SYM

We study the form factors of the Konishi operator, the prime example of non-protected operators in N=4 SYM theory, via the on-shell unitarity methods. Since the Konishi operator is not protected by supersymmetry, its form factors share many features with those in QCD, such as the occurrence of rational terms and of UV divergences that require renormalization. A subtle point is that this operator depends on the spacetime dimension. This requires a modification when calculating its form factors via unitarity methods. We derive a rigorous prescription that implements this modification to all loop orders and obtain the two-point form factor up to two-loop order and the three-point form factor to one-loop order. From these form factors, we construct an IR-finite cross section type quantity, namely the inclusive decay rate of the (off-shell) Konishi operator to any final (on-shell) state. Via the optical theorem, it is connected to the imaginary part of the two-point correlation function. We extract the Konishi anomalous dimension up to two-loop order from it.

==> picturemacro.tex <==
\makeatletter

%% Form factor diagrams
% xkeyval definitions
\define@boolkey{FDff}{oneloop}[true]{}
\define@boolkey{FDff}{twoloop}[true]{}
% \define@boolkey{FDff}{black}[true]{}
% \define@boolkey{FDff}{blue}[true]{}
% \define@boolkey{FDff}{green}[true]{}
\define@boolkey{FDff}{reflected}[true]{}
\define@boolkey{FDff}{fancy}[true]{}
% \define@boolkey{FDff}{small}[true]{}
% \define@key{FDff}{loops}%
%  {\def\FDffloops{#1}}%
\define@key{FDff}{legs}%
 {\def\FDfflegs{#1}}%
\define@key{FDff}{scaled}%
 {\def\FDffscaled{#1}}%
\presetkeys{FDff}{%
% loops=0,%
scaled=1,
legs=2,%
reflected=false,%
fancy=false,%
oneloop=false,%
twoloop=false%
% red=false,%
% bottomleglabel=$\phantom{0}$%
}{}
% Makro / FeynMP definitions
\newcommand*\FDff[1][]{%
 \setkeys{FDff}{#1}%
% 
\setlength{\unitlength}{\FDffscaled mm}%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-8\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(1,1)(1,1){%
\scalebox{1}{%
\fmfstraight%
\begin{fmfchar*}(25,14)%
\expandafter\fmfcmd{%
dash_len := 0.5; 
newinternal numeric loops,legs,scald;
legs:=\FDfflegs;
scald:=\FDffscaled;
% loops:=\FDffloops;
}%
% \begin{fmfshrink}{1}
% outgoing
\ifKV@FDff@reflected
\fmfright{vq}
\fmfleftn{vp}{\FDfflegs}
\else
\fmfleft{vq}
\fmfrightn{vp}{\FDfflegs}
\fi
% internal lines left
\fmf{dbl_plain,tension=legs}{vq,v1}
% internal lines right
\ifKV@FDff@fancy
\fmf{plain}{v1,vp1}
\begin{fmffor}{n}{2}{1}{\FDfflegs-2}
\fmf{phantom}{v1,vp[n]}
\end{fmffor}
\begin{fmffor}{n}{\FDfflegs-1}{1}{\FDfflegs}
\fmf{plain}{v1,vp[n]}
\end{fmffor}
\else
\begin{fmffor}{n}{1}{1}{\FDfflegs}
\fmf{plain}{v1,vp[n]}
\end{fmffor}
\fi
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertq, vertpone, vertptwo, vertone; vertone = vloc(__v1); vertq = vloc(__vq); vertpone = vloc(__vp1); vertptwo = vloc(__vp2);}
 % lines
%  \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
%  \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
%  \fmfi{plain}{(vertpone){dir -170}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
%  \fmfi{plain}{(vertptwo){dir 170}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 % blobs
%  \fmfiv{label=$\cF^{(1)}_{\cO}$,l.d=0,l.a=0}{vertone}
 % labels external states
%  \ifKV@FDff@spacetime
%  \fmfiv{label=$\scriptstyle q$}{vertq}
%  \fmfiv{label=$\scriptstyle p_1$}{vertpone}
%  \fmfiv{label=$\scriptstyle p_2$}{vertptwo}
% \else\fi
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-45}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-60}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-75}{vertone}
% 
% \ifKV@FDff@flavour
%  \fmfiv{label=$\scriptstyle K$}{verttwo+(26,14)}
%  \fmfiv{label=$\scriptstyle I$}{verttwo+(-16,14)}
%  \fmfiv{label=$\scriptstyle L$}{verttwo+(26,-14)}
%  \fmfiv{label=$\scriptstyle J$}{verttwo+(-16,-14)}
% \else\fi
% 
% BLOB
  \fmfiv{decor.shape=circle,decor.filled=60,decor.size=30*scald}{vertone}
\ifKV@FDff@fancy
  \fmfiv{decor.shape=circle,decor.filled=0,decor.size=30*scald,label=$\ncsusyF_n$,l.d=0}{vertone}
  \ifKV@FDff@reflected
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=180}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=190}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=200}{vertone}
  \else
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=0}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=-10}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=-20}{vertone}
  \fi
\else\fi  
\ifKV@FDff@oneloop
  \fmfiv{decor.shape=circle,decor.filled=0,decor.size=15*scald}{vertone}
\else\fi
\ifKV@FDff@twoloop
\fmfcmd{fill (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(6*scald,0))) withcolor white;
draw (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(6*scald,0))) withcolor black;}
\fmfcmd{fill (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(-6*scald,0))) withcolor white;
draw (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(-6*scald,0))) withcolor black;}
%   \fmfiv{decor.shape=circle,decor.filled=0,decor.size=11}{vertone+(7,0)}
%   \fmfiv{decor.shape=circle,decor.filled=0,decor.size=11}{vertone+(-7,0)}
 \else\fi
% \end{fmfshrink}
\end{fmfchar*}%
\fmfcurved
}}}%
}




%% in-line diagrams
% xkeyval definitions
\define@boolkey{FDinline}{cutlabels}[true]{}
\define@boolkey{FDinline}{bubble}[true]{}
\define@boolkey{FDinline}{bubblethree}[true]{}
\define@boolkey{FDinline}{bubbletwoone}[true]{}
\define@boolkey{FDinline}{bubbletwoonerev}[true]{}
\define@boolkey{FDinline}{triangle}[true]{}
\define@boolkey{FDinline}{triangletwoone}[true]{}
\define@boolkey{FDinline}{triangletwoonerev}[true]{}
\define@boolkey{FDinline}{trianglethreetop}[true]{}
\define@boolkey{FDinline}{trianglethreebot}[true]{}
\define@boolkey{FDinline}{box}[true]{}
\define@boolkey{FDinline}{rainbow}[true]{}
\define@boolkey{FDinline}{fliprainbow}[true]{}
\define@boolkey{FDinline}{rainbownonplanar}[true]{}
\define@boolkey{FDinline}{fliprainbownonplanar}[true]{}
\define@boolkey{FDinline}{wedgetop}[true]{}
\define@boolkey{FDinline}{wedgebottom}[true]{}
\define@boolkey{FDinline}{itwo}[true]{}
\define@boolkey{FDinline}{fishtop}[true]{}
\define@boolkey{FDinline}{fishbottom}[true]{}
\define@boolkey{FDinline}{fishtopback}[true]{}
\define@boolkey{FDinline}{fishbottomback}[true]{}
\define@boolkey{FDinline}{trianglesubbubbletop}[true]{}
\define@boolkey{FDinline}{trianglesubbubblebottom}[true]{}
\define@boolkey{FDinline}{trianglefishtop}[true]{}
\define@boolkey{FDinline}{trianglefishbottom}[true]{}
\define@boolkey{FDinline}{trianglefishtopback}[true]{}
\define@boolkey{FDinline}{trianglefishbottomback}[true]{}
\define@boolkey{FDinline}{bubblevertical}[true]{}
\define@boolkey{FDinline}{sunrise}[true]{}
\define@boolkey{FDinline}{sunrisethree}[true]{}
\define@boolkey{FDinline}{bubbletriangle}[true]{}
\define@boolkey{FDinline}{doubletrianglethree}[true]{}
\define@boolkey{FDinline}{doubletriangletwo}[true]{}
\define@boolkey{FDinline}{doublebubble}[true]{}
\define@boolkey{FDinline}{boxtriangle}[true]{}
\define@boolkey{FDinline}{trianglebox}[true]{}
\define@boolkey{FDinline}{boxbubble}[true]{}
\define@boolkey{FDinline}{bubblebox}[true]{}
\define@boolkey{FDinline}{masstop}[true]{}
\define@boolkey{FDinline}{massbottom}[true]{}
\define@boolkey{FDinline}{twomomenta}[true]{}
\define@boolkey{FDinline}{momentum}[true]{}
\define@boolkey{FDinline}{momentumarrow}[true]{}
\define@boolkey{FDinline}{altmomentum}[true]{}
\define@boolkey{FDinline}{twolabels}[true]{}
\define@boolkey{FDinline}{threelabels}[true]{}
\define@boolkey{FDinline}{cut}[true]{}
\define@boolkey{FDinline}{big}[true]{}
\define@boolkey{FDinline}{botdoublecut}[true]{}
\define@boolkey{FDinline}{topdoublecut}[true]{}
\define@boolkey{FDinline}{doublecut}[true]{}
\define@boolkey{FDinline}{slashdoublecut}[true]{}
\define@boolkey{FDinline}{bslashdoublecut}[true]{}
\define@boolkey{FDinline}{triplecut}[true]{}
\define@boolkey{FDinline}{alttriplecut}[true]{}
\define@boolkey{FDinline}{quadruplecut}[true]{}
\define@boolkey{FDinline}{splitlabels}[true]{}
\define@key{FDinline}{labelone}%
{\def\FDinlinelabelone{#1}}%
\define@key{FDinline}{labeltwo}%
{\def\FDinlinelabeltwo{#1}}%
\define@key{FDinline}{labelthree}%
{\def\FDinlinelabelthree{#1}}%
\define@key{FDinline}{toplabel}%
{\def\FDinlinetoplabel{#1}}%
\presetkeys{FDinline}{%
cutlabels=false,%
big=false,%
bubble=false,%
bubblethree=false,%
bubbletwoone=false,%
bubbletwoonerev=false,%
triangle=false,%
trianglethreetop=false,%
trianglethreebot=false,%
triangletwoone=false,%
triangletwoonerev=false,%
box=false,%
rainbow=false,%
fliprainbow=false,%
rainbownonplanar=false,%
fliprainbownonplanar=false,%
wedgetop=false,%
wedgebottom=false,%
itwo=false,%
fishtop=false,%
fishbottom=false,%
fishtopback=false,%
fishbottomback=false,%
trianglesubbubbletop=false,%
trianglesubbubblebottom=false,%
trianglefishtop=false,%
trianglefishbottom=false,%
trianglefishtopback=false,%
trianglefishbottomback=false,%
bubblevertical=false,%
sunrise=false,%
sunrisethree=false,%
massbottom=false,%
masstop=false,%
bubbletriangle=false,%
bubblebox=false,%
boxbubble=false,%
trianglebox=false,%
boxtriangle=false,%
doubletriangletwo=false,%
doubletrianglethree=false,%
doublebubble=false,%
twomomenta=false,%
momentum=false,%
momentumarrow=false,%
altmomentum=false,%
twolabels=false,%
threelabels=false,%
cut=false,%
botdoublecut=false,%
topdoublecut=false,%
doublecut=false,%
slashdoublecut=false,%
bslashdoublecut=false,%
triplecut=false,%
alttriplecut=false,%
quadruplecut=false,%
splitlabels=false,%
toplabel=$\phantom{0}$,%
labelone=\phantom{0},%
labeltwo=\phantom{0},%
labelthree=\phantom{0}%
}{}
% Makro / FeynMP definitions
%straight galeries
\fmfstraight
\newcommand*\FDinline[1][]{%
 \setkeys{FDinline}{#1}%
% 
% BIG
\ifKV@FDinline@big
\unitlength=1mm
\else
\unitlength=0.6mm
\fi
%%% Distances for labels
% TWO LABELS  
 \ifKV@FDinline@twolabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{{\scriptstyle \FDinlinelabelone}}}
 \else\fi
 \else\fi
% THREE LABELS  
 \ifKV@FDinline@threelabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{{\scriptstyle \FDinlinelabelthree}}}
 \else\fi
 \else\fi
%%% diagrams
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-11\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(2,3)(2,3){%
\scalebox{1}{%
\begin{fmfchar*}(30,16)%
\fmfcmd{%
dash_len := 1.5mm; 
}%
% \begin{fmfshrink}{0.5}
\fmfstraight
% cut
\ifKV@FDinline@cut
\fmftop{vtop}
\fmfbottom{vbot}
\fmf{dashes}{vtop,vbot}
\else\fi
% BOX
\ifKV@FDinline@box
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
\fmftop{vt}
\fmfbottom{vb}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0}{v1,v2}
\fmf{plain,right=0}{v1,v3}
% internal lines right
\fmf{plain,tension=0.8}{v2,vp1}
\fmf{plain,tension=0.8}{v3,vp3}
% top and bottom
% \fmf{phantom,tension=1.8}{v2,vt}
% \fmf{phantom,tension=1.8}{v3,vb}
% right corner
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v3}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v3}
\else\fi
\else\fi
% slash double cut
\ifKV@FDinline@slashdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v2,v4}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v3}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=10,label.side=left,left=0,tension=0}{v2,v4}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v3}
\else\fi
\else\fi
% back slash double cut
\ifKV@FDinline@bslashdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0,tension=0}{v3,v4}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=10,label.side=right,right=0,tension=0}{v3,v4}
\else\fi
\else\fi
\fmffreeze
\fmf{plain,left=0}{v2,v4}
\fmf{plain,right=0}{v3,v4}
\fmf{plain,tension=5}{v4,vp2}
\else\fi
% BUBBLE
\ifKV@FDinline@bubble
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l$}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0.7,tension=0}{v1,v2}
\else\fi
\else\fi
\else\fi
% BUBBLETHREE
\ifKV@FDinline@bubblethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l$}{v2,v1}
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0.7,tension=0}{v1,v2}
\else\fi
\else\fi
% two momenta
\ifKV@FDinline@twomomenta
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l_1$}{v2,v1}
\fmf{electron,tension=0,left=0.7,label=$\scriptstyle l_2$}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\fmf{plain,tension=1.5}{v2,vp3}
\else\fi
% BUBBLETWOONE
\ifKV@FDinline@bubbletwoone
% outgoing
\fmfleft{vq,vp3}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\else\fi
% BUBBLETWOONEREV
\ifKV@FDinline@bubbletwoonerev
% outgoing
\fmfleft{vp3,vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\else\fi
% BUBBLE VERTICAL
\ifKV@FDinline@bubblevertical
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{point length(p1)/2 of p1
-- point length(p2)/2 of p2}
\else\fi
% FISHTOP
\ifKV@FDinline@fishtop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% momentumarrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,left=0.7}{v2,v1}
\else\fi
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0.7,label=$\scriptstyle l$}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p1)/2 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
\fmffreeze
% triple cut
\ifKV@FDinline@triplecut
\fmfi{phantom_smallcut}{(point length(p1)/2 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
\fmfi{phantom_smallcut}{subpath (0,0.5*length(p1)) of p1}
\fmfi{phantom_smallcut}{subpath (length(p2),0*length(p2)) of p2}
\else\fi
% cutlabels
\ifKV@FDinline@cutlabels
% \fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$}{(point length(p1)/2 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$}{subpath (0,0.5*length(p1)) of p1}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$}{subpath (length(p2),0*length(p2)) of p2}
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=0,l.d=15}{vert}
\else\fi
\else\fi
% FISHBOTTOMBACK
\ifKV@FDinline@fishbottomback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p2)/2 of p2){dir 90}..{dir 0}(point length(p1) of p1)}
\else\fi
% FISHTOPBACK
\ifKV@FDinline@fishtopback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p1)/2 of p1){dir -90}..{dir 0}(point 0length(p2) of p2)}
\else\fi
% FISHBOTTOM
\ifKV@FDinline@fishbottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% momentumarrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,right=0.7}{v2,v1}
\else\fi
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l$}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p2)/2 of p2){dir 90}..{dir 180}(point 0length(p1) of p1)}
% triple cut
\ifKV@FDinline@triplecut
\fmfi{phantom_smallcut}{(point length(p2)/2 of p2){dir 90}..{dir 180}(point 0length(p1) of p1)}
\fmfi{phantom_smallcut}{subpath (length(p2),0.5*length(p2)) of p2}
\fmfi{phantom_smallcut}{subpath (length(p1),0*length(p1)) of p1}
\else\fi
% cutlabels
\ifKV@FDinline@cutlabels
% \fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$}{(point length(p2)/2 of p2){dir 90}..{dir 180}(point 0length(p1) of p1)}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$}{subpath (length(p2),0.5*length(p2)) of p2}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$}{subpath (length(p1),0*length(p1)) of p1}
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=0,l.d=15}{vert}
\else\fi
\else\fi
% SUNRISE
\ifKV@FDinline@sunrise
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel,tension=0.5}{v1,v2}
\fmf{plain,right=0.7,tension=0.5}{v1,v2}
\fmf{plain,right=0,tension=0}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\fmffreeze
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2}
\else\fi
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,left=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,right=0.7,tension=0}{v1,v2}
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=-15,l.d=18}{vert}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,right=0,tension=0}{v1,v2}
\else\fi
\else\fi
% SUNRISETHREE
\ifKV@FDinline@sunrisethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tension=0.5,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7,tension=0.5}{v1,v2}
\fmf{plain,right=0,tension=0}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\fmf{plain,tension=1.5}{v2,vp3}
\else\fi
% DOUBLEBUBBLE
\ifKV@FDinline@doublebubble
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines middle right
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v2,v3}
\fmf{plain,right=0.7}{v2,v3}
% internal lines right
\fmf{plain,tension=1.5}{v3,vp1}
\fmf{plain,tension=1.5}{v3,vp2}
\else\fi
% BUBBLETRIANGLE
\ifKV@FDinline@bubbletriangle
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2,v2t}
\fmf{plain,right=0.0}{v2,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% TRIANGLE
\ifKV@FDinline@triangle
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\else\fi
\else\fi
\else\fi
% TRIANGLETWOONE
\ifKV@FDinline@triangletwoone
% outgoing
\fmfleft{vq,vp3}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% TRIANGLETWOONEREV
\ifKV@FDinline@triangletwoonerev
% outgoing
\fmfleft{vp3,vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% TRIANGLETHREETOP
\ifKV@FDinline@trianglethreetop
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=0}{v2t,vp2}
\fmf{plain,tension=1.5}{v2b,vp3}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0,label=$\scriptstyle l$,l.d=8,label.side=right}{v2t,v1}
\else\fi
\ifKV@FDinline@altmomentum
\fmf{electron,tension=0,right=0,label=$\scriptstyle l$,l.d=8,label.side=left}{v2b,v1}
\else\fi
% top double cut
\ifKV@FDinline@topdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\fmfposition
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=-5,l.d=30}{vert}
\else\fi
\else\fi
% bottom double cut
\ifKV@FDinline@botdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\else\fi
\else\fi
\else\fi
% TRIANGLETHREEBOT
\ifKV@FDinline@trianglethreebot
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=0}{v2b,vp2}
\fmf{plain,tension=1.5}{v2b,vp3}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=left,l.d=8}{v2b,v1}
\else\fi
\ifKV@FDinline@altmomentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=right,l.d=8}{v2t,v1}
\else\fi
% top double cut
\ifKV@FDinline@topdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\else\fi
\else\fi
% bottom double cut
\ifKV@FDinline@botdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,left=0,tension=0}{v1,v2b}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\fmfposition
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.a=5,l.d=30}{vert}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\else\fi
\else\fi
\else\fi
% DOUBLETRIANGLETHREE
\ifKV@FDinline@doubletrianglethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2m,vp2}
\fmf{plain,tension=2}{v2b,vp3}
\else\fi
% DOUBLETRIANGLETWO
\ifKV@FDinline@doubletriangletwo
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines right
\ifKV@FDinline@masstop
\fmf{double,tension=2}{v2t,vp1}
\else
\fmf{plain,tension=2}{v2t,vp1}
\fi
\ifKV@FDinline@massbottom
\fmf{double,tension=2}{v2b,vp3}
\else
\fmf{plain,tension=2}{v2b,vp3}
\fi
\fmf{phantom,tension=2}{v2m,vp2}
\else\fi
% ITWO
\ifKV@FDinline@itwo
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0,right=0.5}{v2t,v2b}
\fmf{plain,tension=0,left=0.5}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% RAINBOW
\ifKV@FDinline@rainbow
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,tension=0.8,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0,tension=0.8}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=right,l.d=8}{v2t,v1}
\else\fi
% momentum arrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,left=0}{v2t,v1}
\else\fi
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0}{v3t,v3b}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,right=0,tension=0}{v2b,v3b}
\else\fi
\else\fi
% alternative triple cut
\ifKV@FDinline@alttriplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
% quadruple cut
\ifKV@FDinline@quadruplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=right,right=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% \fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
% \fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
 \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
 \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
\else\fi
% FLIPPED RAINBOW
\ifKV@FDinline@fliprainbow
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{phantom,left=0.0,tension=0.8}{vq,v2t}
\fmf{phantom,right=0.0,tension=0.8}{vq,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines middle left
\fmf{phantom,left=0.0,tension=0.0001,tag=1}{v1,v3t}
\fmf{phantom,right=0.0,tension=0.0001}{v1,v3b}
\fmf{plain,left=0.0,tension=0.00005}{v1,v2t}
\fmf{plain,right=0.0,tension=0.00005}{v1,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=left,l.d=8}{v2t,v1}
\else\fi
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0,tag=1}{v3t,v3b}
% internal lines right
\fmf{plain,tension=1.8}{v3t,vp1}
\fmf{plain,tension=1.8}{v3b,vp2}
% double line
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v3t)}
\fmfiset{p2}{vpath1(__v3t,__v3b)}
% \fmfi{double}{point 0*length(p1)/2 of p1 -- point length(p2)/2 of p2}
\fmfi{double}{point 0*length(p1)/2 of p1 -- 0.5*((point length(p2)/2 of p2)+(point 0*length(p1)/2 of p1))}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=13,label.side=right,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=right,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,right=0,tension=0}{v2b,v3b}
\else\fi
\else\fi
% alternative triple cut
\ifKV@FDinline@alttriplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=13,label.side=left,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
% quadruple cut
\ifKV@FDinline@quadruplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
\else\fi
% BOXTRIANGLE
\fmfstraight
\ifKV@FDinline@boxtriangle
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines middle right
\fmf{plain,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v3t,v3m}
% internal lines right
\fmf{plain,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% TRIANGLEBOX
\fmfstraight
\ifKV@FDinline@trianglebox
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,tension=0}{v2t,v2m}
% internal lines middle right
\fmf{plain,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v3m,v3b}
% internal lines right
\fmf{plain,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% WEDGETOP
\ifKV@FDinline@wedgetop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines middle right
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0}{v2t,v3b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
\else\fi
% WEDGEBOTTOM
\ifKV@FDinline@wedgebottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,tension=0}{v3t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% RAINBOW NONPLANAR
\ifKV@FDinline@rainbownonplanar
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,tension=0.8,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0,tension=0.8}{v1,v2b}
\fmf{plain,tension=0,rubout}{v2t,v3b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=8}{v2t,v1}
\else\fi
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0}{v3t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
\else\fi
% FLIPPED RAINBOW NONPLANAR
\ifKV@FDinline@fliprainbownonplanar
% outgoing
\fmfleft{vp1}
\fmfright{vp2}
\fmftop{vt}
\fmfbottom{vb}
% internal lines left
\fmf{plain,tension=5}{vp1,vl}
% internal lines middle
\fmf{phantom,tension=10}{vt,vta}
\fmf{plain,tension=1}{vta,v1}
\fmf{plain,tension=1}{vba,v1}
\fmf{phantom,tension=10}{vba,vb}
% internal lines middle left
\fmf{plain,tension=1}{vta,vl}
\fmf{plain,tension=1}{vba,vl}
% internal lines middle right
\fmf{plain,tension=1}{vta,vr}
\fmf{plain,tension=1}{vba,vr}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=8,label.side=right}{v1,vta}
\else\fi
% momentum arrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,left=0}{vta,v1}
\else\fi
% internal lines right
\fmf{plain,tension=5}{vr,vp2}
% double line
\fmf{phantom,tension=0,tag=1}{vl,v1}
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__vl,__v1)}
\fmfi{double}{subpath (length(p1),0.6*length(p1)) of p1}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vta}
\fmf{phantom_smallcut,right=0,tension=0}{vr,vba}
\fmf{phantom_smallcut,right=0,tension=0}{vl,vba}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=right,left=0,tension=0}{v1,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=left,right=0,tension=0}{vr,vba}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=right,right=0,tension=0}{vl,vba}
\else\fi
\else\fi
% alternative triple cut
\ifKV@FDinline@alttriplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vba}
\fmf{phantom_smallcut,right=0,tension=0}{vta,vl}
\fmf{phantom_smallcut,right=0,tension=0}{vta,vr}
% cutlabels
\ifKV@FDinline@cutlabels
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
%  \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.a=+25,l.d=7}{vert}
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=-25,l.d=7}{vert}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,left=0,tension=0}{v1,vba}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=right,right=0,tension=0}{vr,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=left,right=0,tension=0}{vl,vta}
\else\fi
\else\fi
% quadruple cut
\ifKV@FDinline@quadruplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vta}
\fmf{phantom_smallcut,right=0,tension=0}{v1,vba}
\fmf{phantom_smallcut,right=0,tension=0}{vta,vr}
\fmf{phantom_smallcut,right=0,tension=0}{vba,vl}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v1,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=left,right=0,tension=0}{v1,vba}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=left,right=0,tension=0}{vta,vr}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=left,right=0,tension=0}{vba,vl}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vta}
\fmf{phantom_smallcut,right=0,tension=0}{v1,vba}
% \fmf{phantom_smallcut,right=0,tension=0}{vta,vr}
% \fmf{phantom_smallcut,right=0,tension=0}{vba,vl}
% cutlabels
\ifKV@FDinline@cutlabels
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=right,left=0,tension=0}{v1,vta}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v1,vba}
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.a=+25,l.d=7}{vert}
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=-25,l.d=7}{vert}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=left,right=0,tension=0}{vta,vr}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=left,right=0,tension=0}{vba,vl}
\else\fi
\else\fi
\else\fi
% TRIANGLEFISHTOP
\ifKV@FDinline@trianglefishtop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 2length(p1)/3 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
\else\fi
% TRIANGLEFISHBOTTOMBACK
\ifKV@FDinline@trianglefishbottomback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 2length(p2)/3 of p2){dir 30}..{dir -70}(point 0length(p2) of p2)}
\else\fi
% TRIANGLEFISHTOPBACK
\ifKV@FDinline@trianglefishtopback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 1length(p1)/3 of p1){dir -30}..{dir 70}(point length(p1) of p1)}
\else\fi
% TRIANGLEFISHBOTTOM
\ifKV@FDinline@trianglefishbottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 1length(p2)/3 of p2){dir 90}..{dir 180}(point length(p2) of p2)}
\else\fi
% TRIANGLESUBBUBBLEBOTTOM
\ifKV@FDinline@trianglesubbubblebottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\ifKV@FDinline@masstop
\fmf{double,tension=2}{v2t,vp1}
\else
\fmf{plain,tension=2}{v2t,vp1}
\fi
\ifKV@FDinline@massbottom
\fmf{double,tension=2}{v2b,vp2}
\else
\fmf{plain,tension=2}{v2b,vp2}
\fi
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point length(p2) of p2){dir 0}..{dir -70}(point 0length(p2) of p2)}
\else\fi
% TRIANGLESUBBUBBLETOP
\ifKV@FDinline@trianglesubbubbletop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\ifKV@FDinline@masstop
\fmf{double,tension=2}{v2t,vp1}
\else
\fmf{plain,tension=2}{v2t,vp1}
\fi
\ifKV@FDinline@massbottom
\fmf{double,tension=2}{v2b,vp2}
\else
\fmf{plain,tension=2}{v2b,vp2}
\fi
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 0length(p1) of p1){dir 0}..{dir 70}(point length(p1) of p1)}
\else\fi
% BOXBUBBLE
\fmfstraight
\ifKV@FDinline@boxbubble
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
\fmf{phantom,right=0.0}{v1,v2b}
\fmf{plain,right=0.7,tension=0}{v1,v2m}
% internal lines middle right
\fmf{plain,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{phantom,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,tension=0}{v3t,v3m}
% internal lines right
\fmf{plain,tension=2}{v3t,vp1}
\fmf{plain,tension=0}{v2m,vp3}
\fmf{phantom,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% BUBBLEBOX
\fmfstraight
\ifKV@FDinline@bubblebox
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,tension=0}{v1,v2m}
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v3m,v3b}
% internal lines right
\fmf{plain,tension=0}{v2m,vp1}
\fmf{phantom,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% LABELS
%
% THREE LABELS  
 \ifKV@FDinline@threelabels
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertpone, vertptwo, vertpthree; vertpone = vloc(__vp1); vertptwo = vloc(__vp2); vertpthree = vloc(__vp3);}
 % labels
 \fmfiv{label=$\scriptstyle \FDinlinelabelone$,l.a=0,l.d=4}{vertpone}
 \fmfiv{label=$\scriptstyle \FDinlinelabeltwo$,l.a=0,l.d=4}{vertptwo}
 \ifKV@FDinline@splitlabels
 \fmfiv{label=$\scriptstyle \FDinlinelabelthree$,l.a=180,l.d=4}{vertpthree}
 \else
 \fmfiv{label=$\scriptstyle \FDinlinelabelthree$,l.a=0,l.d=4}{vertpthree}
 \fi
 \else\fi
%
% TWO LABELS  
 \ifKV@FDinline@twolabels
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertpone, vertptwo, vertpthree; vertpone = vloc(__vp1); vertptwo = vloc(__vp2);}
 % labels
 \ifKV@FDinline@splitlabels
 \fmfiv{label=$\scriptstyle \FDinlinelabelone$,l.a=180,l.d=4}{vertpone}
 \fmfiv{label=$\scriptstyle \FDinlinelabeltwo$,l.a=0,l.d=4}{vertptwo}
 \else
 \fmfiv{label=$\scriptstyle \FDinlinelabelone$,l.a=0,l.d=4}{vertpone}
 \fmfiv{label=$\scriptstyle \FDinlinelabeltwo$,l.a=0,l.d=4}{vertptwo}
 \fi
 \else\fi
% \end{fmfshrink}
\end{fmfchar*}%
% Set back to curved galeries
 \fmfcurved
}}}%
%%% Distances for labels
% TWO LABELS  
 \ifKV@FDinline@twolabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{{\scriptstyle \FDinlinelabeltwo}}}
\else
\ensuremath{\phantom{\frac{\scriptstyle \FDinlinelabelone}{\scriptstyle \FDinlinelabeltwo}}}
\fi\else\fi
% THREE LABELS  
 \ifKV@FDinline@threelabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{\frac{\scriptstyle \FDinlinelabelone}{\scriptstyle \FDinlinelabeltwo}}}
\else
\ensuremath{\phantom{\frac{\scriptstyle \FDinlinelabelone}{\frac{\scriptstyle \FDinlinelabelone}{\scriptstyle \FDinlinelabelthree}}}}
 \fi\else\fi
}


%% in-line diagrams
% xkeyval definitions
\define@boolkey{FDdimred}{zigzagbubble}[true]{}
\define@boolkey{FDdimred}{scalarbubble}[true]{}
\define@boolkey{FDdimred}{gluonbubble}[true]{}
\define@boolkey{FDdimred}{zigzagfermion}[true]{}
\define@boolkey{FDdimred}{scalarfermion}[true]{}
\define@boolkey{FDdimred}{gluonfermion}[true]{}
\define@boolkey{FDdimred}{bubble}[true]{}
\define@boolkey{FDdimred}{triangle}[true]{}
\define@boolkey{FDdimred}{cut}[true]{}
\define@key{FDdimred}{toplabel}%
{\def\FDdimredtoplabel{#1}}%
\define@key{FDdimred}{topleglabel}%
{\def\FDdimredtopleglabel{#1}}%
\define@key{FDdimred}{bottomleglabel}%
{\def\FDdimredbottomleglabel{#1}}%
\presetkeys{FDdimred}{%
zigzagbubble=false,%
scalarbubble=false,%
gluonbubble=false,%
zigzagfermion=false,%
scalarfermion=false,%
gluonfermion=false,%
bubble=false,%
triangle=false,%
cut=false,%
toplabel=$\phantom{0}$,%
topleglabel=$\phantom{0}$,%
bottomleglabel=$\phantom{0}$%
}{}
% Makro / FeynMP definitions
\newcommand*\FDdimred[1][]{%
 \setkeys{FDdimred}{#1}%
% 
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-8\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(1,0)(1,0){%
\scalebox{1}{%
\begin{fmfchar*}(30,16)%
\fmfcmd{%
dash_len := 1.6mm; 
}%
\begin{fmfshrink}{0.5}
% cut
\ifKV@FDdimred@cut
\fmftop{vtop}
\fmfbottom{vbot}
\fmf{dashes}{vtop,vbot}
\else\fi
% SCALARBUBBLE
\ifKV@FDdimred@scalarbubble
% outgoing
\fmfleft{vq1,vq2}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=1}{vq1,v1}
\fmf{plain,tension=1}{vq2,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1}{v2,vp1}
\fmf{plain,tension=1}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% GLUONBUBBLE
\ifKV@FDdimred@gluonbubble
% outgoing
\fmfleft{vq1,vq2}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=1}{vq1,v1}
\fmf{plain,tension=1}{vq2,v1}
% internal lines middle
\fmf{wiggly,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{wiggly,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1}{v2,vp1}
\fmf{plain,tension=1}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% ZIGZAGBUBBLE
\ifKV@FDdimred@zigzagbubble
% outgoing
\fmfleft{vq1,vq2}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=1}{vq1,v1}
\fmf{plain,tension=1}{vq2,v1}
% internal lines middle
\fmf{zigzag,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{zigzag,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1}{v2,vp1}
\fmf{plain,tension=1}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% BUBBLE
\ifKV@FDdimred@bubble
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=2}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1.2}{v2,vp1}
\fmf{plain,tension=1.2}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% TRIANGLE
\ifKV@FDdimred@triangle
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=2}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDdimredtoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.2}{v2t,vp1}
\fmf{plain,tension=1.2}{v2b,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% ZIGZAGFERMION
\ifKV@FDdimred@zigzagfermion
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{zigzag,tension=2}{vq,v1}
% internal lines right
\fmf{dashes,tension=1}{v1,vp1}
\fmf{dashes,tension=1}{v1,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% SCALARFERMION
\ifKV@FDdimred@scalarfermion
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=2}{vq,v1}
% internal lines right
\fmf{dashes,tension=1}{v1,vp1}
\fmf{dashes,tension=1}{v1,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% GLUONFERMION
\ifKV@FDdimred@gluonfermion
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{photon,tension=2}{vq,v1}
% internal lines right
\fmf{dashes,tension=1}{v1,vp1}
\fmf{dashes,tension=1}{v1,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
\end{fmfshrink}
\end{fmfchar*}%
}}}%
}


%% flow diagrams
% xkeyval definitions
\define@boolkey{FDflow}{spacetime}[true]{}
\define@boolkey{FDflow}{flavour}[true]{}
\define@boolkey{FDflow}{black}[true]{}
\define@boolkey{FDflow}{blue}[true]{}
\define@boolkey{FDflow}{green}[true]{}
\define@boolkey{FDflow}{red}[true]{}
\define@boolkey{FDflow}{fermion}[true]{}
\define@boolkey{FDflow}{twopoint}[true]{}
\define@boolkey{FDflow}{cutleft}[true]{}
\define@boolkey{FDflow}{cutright}[true]{}
\define@boolkey{FDflow}{cutmiddle}[true]{}
% \define@key{FDdimred}{bottomleglabel}%
% {\def\FDdimredbottomleglabel{#1}}%
\presetkeys{FDflow}{%
flavour=false,%
spacetime=false,%
black=false,%
blue=false,%
green=false,%
red=false,%
fermion=false,%
twopoint=false,%
cutmiddle=false,%
cutright=false,%
cutleft=false,%
% bottomleglabel=$\phantom{0}$%
}{}
% Makro / FeynMP definitions
\newcommand*\FDflow[1][]{%
 \setkeys{FDflow}{#1}%
%
\fmfstraight
%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-10\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(0,3)(4,3){%
\scalebox{1}{%
\begin{fmfchar*}(25,14)%
\fmfcmd{%
dash_len := 1.6mm; 
}%
\begin{fmfshrink}{1}
% FERMIONS
\ifKV@FDflow@fermion
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{dbl_plain,tension=10}{vq,v1}
% internal lines middle
\fmf{phantom,left=1.0}{v1,v2}
\fmf{phantom,right=1.0}{v1,v2}
% internal lines right
\fmf{phantom,tension=1.0}{v2,vp1}
\fmf{phantom,tension=1.0}{v2,vp3}
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertq, vertpone, vertptwo, vertpthree, vertone, verttwo; vertone = vloc(__v1); verttwo = vloc(__v2); vertq = vloc(__vq); vertpone = vloc(__vp1); vertptwo = vloc(__vp2); vertpthree = vloc(__vp3);}
 % lines
 \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain}{(vertpone){dir -170}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertptwo){dir -180}..{dir 0}(verttwo+(20,0))}
 \fmfi{plain}{(vertpthree){dir 170}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
% TWO-POINT FUNCTION
 \else
 \ifKV@FDflow@twopoint
 % outgoing
\fmfleft{vq1}
\fmfright{vq2}
% internal lines left
\fmf{dbl_plain,tension=10}{vq1,v1}
% internal lines middle
\fmf{phantom,left=1.0}{v1,v2}
\fmf{phantom,right=1.0}{v1,v2}
\fmf{phantom,left=1.0}{v2,v3}
\fmf{phantom,right=1.0}{v2,v3}
% internal lines right
\fmf{dbl_plain,tension=10}{v3,vq2}
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertqone,  vertqtwo, vertone, verttwo, vertthree; vertqone = vloc(__vq1); vertone = vloc(__v1);verttwo = vloc(__v2);vertthree = vloc(__v3); vertqtwo = vloc(__vq2); }
 % lines
 \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain}{(vertthree){dir 120}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertthree){dir -120}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 % SCALARS 
 \else
 % outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{dbl_plain,tension=10}{vq,v1}
% internal lines middle
\fmf{phantom,left=1.0}{v1,v2}
\fmf{phantom,right=1.0}{v1,v2}
% internal lines right
\fmf{phantom,tension=1.0}{v2,vp1}
\fmf{phantom,tension=1.0}{v2,vp2}
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertq, vertpone, vertptwo, vertone, verttwo; vertone = vloc(__v1); verttwo = vloc(__v2); vertq = vloc(__vq); vertpone = vloc(__vp1); vertptwo = vloc(__vp2);}
 % lines
 \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain}{(vertpone){dir -170}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertptwo){dir 170}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 \fi
 \fi
 % blobs
%  \fmfiv{label=$\cF^{(1)}_{\cO}$,l.d=0,l.a=0}{vertone}
 % labels external states
 \ifKV@FDflow@spacetime
 \ifKV@FDflow@twopoint
 \fmfiv{label=$\scriptstyle q$}{vertqone}
 \fmfiv{label=$\scriptstyle q$}{vertqtwo}
 \else
 \fmfiv{label=$\scriptstyle q$}{vertq}
 \fmfiv{l.a=0,label=$\scriptstyle p_1$}{vertpone}
 \fmfiv{l.a=0,label=$\scriptstyle p_2$}{vertptwo}
 \ifKV@FDflow@fermion
 \fmfiv{label=$\scriptstyle p_3$}{vertpthree}
\else\fi
\fi
\else\fi
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-45}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-60}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-75}{vertone}
% 
\ifKV@FDflow@flavour
 \fmfiv{label=$\scriptstyle I$}{verttwo+(-16,14)}
 \fmfiv{label=$\scriptstyle J$}{verttwo+(-16,-14)}
 \ifKV@FDflow@fermion 
 \fmfiv{l.a=0,label=$\scriptstyle K$}{vertpone}
 \fmfiv{l.a=0,label=$\scriptstyle A$}{vertptwo}
 \fmfiv{l.a=0,label=$\scriptstyle B$}{vertpthree}
 \else
 \ifKV@FDflow@twopoint
 \fmfiv{label=$\scriptstyle K$}{verttwo+(+16,14)}
 \fmfiv{label=$\scriptstyle L$}{verttwo+(+16,-14)}
 \else
 \fmfiv{l.a=0,label=$\scriptstyle K$}{vertpone}
 \fmfiv{l.a=0,label=$\scriptstyle L$}{vertptwo}
 \fi
 \fi
\else\fi
% 
\ifKV@FDflow@black
 \fmfiv{decor.shape=circle,decor.filled=60,decor.size=40}{verttwo}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(7,7)}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(-7,7)}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(7,-7)}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(-7,-7)}
\else\fi
% 
\ifKV@FDflow@blue
  \fmfiv{decor.shape=circle,decor.filled=20,decor.size=40}{verttwo}
 \fmfdraw
 \ifKV@FDflow@fermion 
 \fmfi{plain,fore=blue}{(verttwo+(0,-8)){dir 90}..{dir 0}(verttwo+(20,0))}
 \else\fi
 \fmfi{plain,fore=blue}{(verttwo+(-20/sqrt(2),20/sqrt(2))){dir -45}..{dir 45}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain,fore=blue}{(verttwo+(-20/sqrt(2),-20/sqrt(2))){dir 45}..{dir -45}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
\else\fi
% 
\ifKV@FDflow@red
  \fmfiv{decor.shape=circle,decor.filled=20,decor.size=40}{verttwo}
 \fmfdraw
 \ifKV@FDflow@fermion 
 \fmfi{plain,fore=red}{(verttwo+(11,0)){dir 180}..{dir 0}(verttwo+(20,0))}
 \else\fi
 \fmfi{plain,fore=red}{(verttwo+(-20/sqrt(2),20/sqrt(2))){dir -45}..{dir -135}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain,fore=red}{(verttwo+(20/sqrt(2),20/sqrt(2))){dir -135}..{dir -45}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
\else\fi
% 
\ifKV@FDflow@green
  \fmfiv{decor.shape=circle,decor.filled=20,decor.size=40}{verttwo}
 \fmfdraw
 \ifKV@FDflow@fermion 
 \fmfi{plain,fore=green}{(verttwo+(10/sqrt(2),-10/sqrt(2))){dir +45}..{dir 0}(verttwo+(20,0))}
 \else\fi
 \fmfi{plain,fore=green}{(verttwo+(-20/sqrt(2),20/sqrt(2))){dir -45}..{dir -45}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain,fore=green}{(verttwo+(-20/sqrt(2),-20/sqrt(2))){dir 45}..{dir 45}(verttwo-(2/sqrt(2),2/sqrt(2)))}
 \fmfi{plain,fore=green}{(verttwo+(2/sqrt(2),2/sqrt(2))){dir 45}..{dir 45}(verttwo+(20/sqrt(2),20/sqrt(2)))}
\else\fi
\fmftop{vt}
\fmfbottom{vb}
\fmfposition
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair verttop, vertbot; verttop = vloc(__vt); vertbot = vloc(__vb); }
\ifKV@FDflow@cutmiddle
\fmfi{dashes}{(verttop+(0,8))--(vertbot+(0,-8))}
\else\fi
\ifKV@FDflow@cutleft
\fmfi{dashes}{(verttop+(-11,8))--(vertbot+(-11,-8))}
\else\fi
\ifKV@FDflow@cutright
\fmfi{dashes}{(verttop+(11,8))--(vertbot+(11,-8))}
\else\fi
\end{fmfshrink}
\end{fmfchar*}%
}}}%
}











\makeatother

\newcommand{\initialisepictures}{
\fmfcmd{%
thin := 1pt; % dimension of the lines
thick := 2thin;
arrow_len := 3mm;
arrow_ang := 15;
curly_len := 3mm;
dash_len :=0.5; % 'photon' lines
% dash_space := 4mm;
dot_len := 0.75mm; % 'photon' lines
wiggly_len := 2mm; % 'photon' lines
wiggly_slope := 60;
zigzag_len := 2mm;
zigzag_width := 2thick;
decor_size := 5mm;
dot_size := 2thick;
}
\fmfcmd{%
marksize=7mm;
%
def draw_cut(expr p,a) =
  begingroup
    save t,tip,dma,dmb; pair tip,dma,dmb;
    t=arctime a of p;
    tip =marksize*unitvector direction t of p;
    dma =marksize*unitvector direction t of p rotated -90;
    dmb =marksize*unitvector direction t of p rotated 90;
    linejoin:=beveled;
%     draw (-.5dma.. .5tip-- -.5dmb) shifted point t of p;
%     drawoptions(dashed evenly);
    drawoptions(dashed dashpattern(on 6bp off 12bp on 6bp));
    draw ((-.5dma.. -.5dmb) shifted point t of p);
    drawoptions();
  endgroup
enddef;
%
style_def phantom_cut expr p =
    save amid;
    amid=.5*arclength p;
    draw_cut(p, amid);
    draw p;
enddef;
}
\fmfcmd{%
smallmarksize=4mm;
%
def draw_smallcut(expr p,a) =
  begingroup
    save t,tip,dma,dmb; pair tip,dma,dmb;
    t=arctime a of p;
    tip =smallmarksize*unitvector direction t of p;
    dma =smallmarksize*unitvector direction t of p rotated -90;
    dmb =smallmarksize*unitvector direction t of p rotated 90;
    linejoin:=beveled;
%     draw (-.5dma.. .5tip-- -.5dmb) shifted point t of p;
%     drawoptions(dashed evenly);
    drawoptions(dashed dashpattern(on 2bp off 2bp on 2bp) withcolor red);
    draw ((-.5dma.. -.5dmb) shifted point t of p);
    drawoptions();
  endgroup
enddef;
%
style_def phantom_smallcut expr p =
    save amid;
    amid=.5*arclength p;
    draw_smallcut(p, amid);
    draw p;
enddef;
}
}
